DoseGNN: Improving the Performance of Deep Learning Models in Adaptive Dose-Volume Histogram Prediction through Graph Neural Networks

Dose-Volume Histogram (DVH) prediction is fundamental in radiation therapy that facilitate treatment planning, dose evaluation, plan comparison and etc. It helps to increase the ability to deliver precise and effective radiation treatments while managing potential toxicities to healthy tissues as needed to reduce the risk of complications. This paper extends recently disclosed research findings presented on AAPM (AAPM 65th Annual Meeting $\&$ Exhibition) and includes necessary technique details. The objective is to design efficient deep learning models for DVH prediction on general radiotherapy platform equipped with high performance CBCT system, where input CT images and target dose images to predict may have different origins, spacing and sizes. Deep learning models widely-adopted in DVH prediction task are evaluated on the novel radiotherapy platform, and graph neural networks (GNNs) are shown to be the ideal architecture to construct a plug-and-play framework to improve predictive performance of base deep learning models in the adaptive setting.

==> 2_backg.tex <==
In this section, we introduce useful concepts. and then reveal the trade-off between the expressivity and stability in GNNs enhanced by graph canonization. Let $G = (V, E, c)$ denote a colored graph of $n$ nodes, where $V = \{v_1, v_2, ..., v_n\}$ is the set of nodes, $ E \in V \times V$ is the set of edges, and the function $c: V \to \mathbb{N}$ associates to each node an integer color (node type). The edge information is always expressed as an adjacency matrix $A \in \{0, 1\}^{n \times n} $ such that $A_{i,j} = 1$ iff edge $(i,j) \in E$.

A \textit{colouring} of $G$ is a surjective function from the node set $V$ onto a set of $k$ integers. In this paper, We use "colouring" to denote both the image of this surjective function (i.e. set of integers). A colouring is discrete if $k=n$,  then each cell (i.e. set of nodes $v \in V$ with the same image) is a singleton. 


\subsection{Graph Distance and Stable GNNs} 
Let $\pi: V \to V$ be a permutation operation on the node set $V$. We denote by $v^{\pi}$ the image of any node $v \in V$, then $\pi(G)$ (i.e. permutation operation on a graph $G$) generates another colored graph $\pi(G) = G^{\pi} = (V, E^{\pi}, c^{\pi})$ such that (1) $(v_{1}^{\pi}, v_{2}^{\pi}) \in E^{\pi}$ iff $(v_{1}, v_{2}) \in E$ (i.e. $A^{\pi}_{v_{1}, v_{2}} = A_{v_{1}, v_{2}}$) and (2) $c^{\pi}(v^{\pi}) = c(v)$. Each permutation operation $\pi$ associates to a $n$-dimension permutation matrix $P^{\pi}$ in $\{0, 1\}^{n \times n}$, where each row and each column has only one single $1$. All the permutation operation $\pi$ on graphs of $n$ nodes formulate a permutation group $\Pi(n)$. 

Given two $n$-size graphs $G_{1} = (V_{1}, E_{1}, c_{1})$, $G_{2} = (V_{2}, E_{2}, c_{2})$ and their corresponding adjacency matrix $A_{1}$ and $A_{2}$, there exists a permutation operation $\pi^{*} \in \Pi(n)$ associates to the permutation matrix $P^{*}$ that best aligns the graph structures and the node colors (i.e. node features),
\begin{align*}
    P^{*} = \textit{argmin}_{P \in \Pi} || A_{1} - PA_{2}P^{T}||_{F} 
    + \sum^{n}_{i}c_{1}(i) != c_{2}(\pi(i))
\end{align*}
The distance between two graphs is thus characterized as $d(G_{1}, G_{2}) = || A_{1} - P^{*}A_{2}P^{*T}||_{F} + \sum_{i}c_{1}(i) != c_{2}(\pi^{*}(i))$, which measures the similarity of two graphs of the same size. 

Equipped with the notion of graph distance, we characterize the the stability of GNN models. The GNN model provides graph representation vector based on adjacency information and node features, then we express it as $g(A, X)$, where $X$ is a $2$-dimension tensor of one-hot features of node colors. Unless specified, following theoretical analysis assumes a GNN model consists of several message passing (MP) layers and a sum readout layer. 

\begin{defi}
\label{def:2}
(Stability). A GNN model $g$ is claimed to be stable under $X$, if there exists a constant $C > 0$, for any two graphs $G_{1}$, $G_{2}$, $g$ satisfies $|| g(A_{1}, X_{1})- g(A_{2},X_{2})||_{2} \leq C d(G_{1},G_{2})$.
\end{defi}

In analog to \cite{wang2022equivariant}, the stability of a GNN model guarantees that similar graphs in the graph distance space will be mapped to similar representations in the vectorial space. Hence, it will provide good generalization ability to apply GNNs on unseen graphs. Overall, the stability and expressivity are two fundamental design principles of GNN architectures. The stability helps to bound the gap between the representations of an unseen testing graph and a similar but different training graph, while the higher expressivity enables GNNs to recognize more graph structures.

\subsection{GNNs with Graph Canonization}
\begin{figure}[t]
\begin{center}
%\vskip -0.15in
\centerline{\includegraphics[width=0.7\textwidth]{overall_arch.pdf}}
%\vspace{-10pt}
\vspace{-6pt}
\caption{Overview of graph canonization techniques in the design of GNNs. Graph canonization improves the expressivity of GNNs at the cost of stability. Consequently, universal graph canonization is proposed to alleviate the problem .}
\label{fig:fig1}
\vskip -0.35in
\end{center}
\end{figure}

Two colored graphs $G_{1}$ and $G_{2}$ of $n $ nodes are isomorphic (denoted by $G_{1} \simeq G_{2}$) if there exists a permutation operation $\pi \in \Pi(n)$ such that $\pi(G_{1}) = G_{2}$. The set all colored graphs isomorphic to $G$ forms it's isomorphism class $ISO(G) = \{G^{'} | G^{'} \simeq G\}$, while an automorphism of $G$ is an isomorphism that maps $G$ onto itself.

\begin{defi}
\label{def:1}
(Graph canonization) Graph canonization $f_{n}$ is a function that maps a colored graph to an isomorphism of the graph itself (a graph in $ISO(G)$) such that $\forall \pi \in \Pi(n)$, $f_{n}(G) = f_{n}(\pi(G))$.
\end{defi}

In other words, graph canonization assigns to each coloured graph an isomorphic coloured graph that is a unique representative of its isomorphism class. The order of nodes $v \in f_{n}(G)$ are denoted as $\rho(v|G)$. Then, the graph canonization provides a unique discrete colouring $\{\rho(v_1|G), \rho(v_2|G), ..., \rho(v_n|G)\}$ as nodes' positions for each isomorphism class $ISO(G)$ to break the symmetry of nodes. 

%Henceforth, we use $P$ to denote a $2$-dimension tensor of one-hot features of this discrete colouring.

\begin{lemma}
\label{lemma:2_4}
    Let $P$ be a $2$-dimension tensor of one-hot features of the discrete colouring generated by an arbitrary graph canonization algorithm. A GNN model $g$ that takes $P$ as nodes' positional encodings maximizes the expressivity, if graph convolution layers of $g$ are injective.
\end{lemma}

\begin{lemma}
\label{lemma:2_3}
    Let $P$ be a $2$-dimension tensor of one-hot features of the discrete colouring generated by a graph canonization algorithm follows the individualization-refinement paradigm. A GNN model $g$ is stable under $X$, and is not stable under $X \oplus P$, where $\oplus$ denotes the concatenation operation.
\end{lemma} 

We prove lemma~\ref{lemma:2_4} and lemma~\ref{lemma:2_3} in Appendix~\ref{sec:appenC}. Graph canonization algorithms that follow the individualization-refinement paradigm ~\cite{grohe2017color} will respect the order of initial node colors/types when breaking ties to introduce the node asymmetry, thus there always exists similar graphs to have complete different discrete colourings as Figure ~\ref{fig:fig2} illustrates. These two lemmas indicate the trade-off of expressivity and stability in GNNs enhanced by graph canonization. Then, graph-canonization-enhanced GNNs (GC-GNNs) can distinguish more graph structures in the training data, yet the ability of generalizing well to unseen testing data is deteriorated to some extend. Hence, we study how to overcome this trade-off in next section. Furthermore, since the graph canonization problem is NP-hard, and practical tools like Nauty~\citep{mckay2014practical} and Bliss ~\citep{junttila2012bliss} for the problem always follow the individualization-refinement paradigm, the trade-off is not generally solvable in practice. 

%Consequently, we characterize a widely applicable sufficient condition to solve the problem for numerous specific scenarios in real world. 

%As non-isomorphic graphs are theoretically distinguishable by generating unique colourings for graphs based on their structures in a permutation-invariant way and then, comparing them, GNNs take discrete colouring $\{\rho(v_1|G), \rho(v_2|G), ..., \rho(v_n|G)\}$ as positional encodings (additional node features) can maximize the expressivity.

==> 4_benchmark.tex <==
%\zehao{
%Please finish the subsection:
%\begin{itemize}
%    \item How to convert circuits to graphs
%    \item how to perform the circuit performance evaluation
%\end{itemize}
%}

%\wdedit{I will add a brief introduction to show Op-Amps are used as open benchmark. Done}



We take operational amplifiers (Op-Amps) to build our open circuit benchmark as they are not only one of the most difficult analog circuits to design in the world, but also are the common benchmarks used by prior arts~\citep{wang2020gcn,li2021circuit, gnn_rl} to evaluate the performance of the proposed methods.
Our benchmark equips with communicative circuit generation and evaluation
capabilities such that it can also be applied to incorporate a broad range of analog circuits for the evaluations of various design automation methods.
To enable such great capabilities, two notable features are proposed and introduced below.

\textbf{Converting Circuits into Graphs}
% Prior arts convert a given analog circuit into a graph in an exact one-to-one mapping manner, i.e., each device corresponds to a graph vertice, and the physical connection between devices is associated with an edge.
% However, this mapping manner has several fatal drawbacks.
% First, it is unscalable, thereby failing to work for large-scale analog circuits with thousands of devices. 
% Second, it introduces cycles into the converted graph as analog circuits often have closed-loop structures.
% Here, 
We leverage an acyclic graph conversion method by abstracting a complex circuit structure to several simple low-level functional sub-structures, which is similar to the standard synthesis of modern digital circuits. 
Such a mapping method is thus scalable to very large-scale analog circuits with thousands of devices while effectively avoiding cycles in graph converting.
To illustrate this general mapping idea, we take the Op-Amps in our benchmark as an example (see the left upper corner in Figure~\ref{fig:over_arcg}). 
For an $N$-stage Op-Amp ($N=2,3$), it consists of $N$ single-stage Op-Amps in the main feedforward path (i.e., from the input direction to the output direction) and several feedback paths (i.e., vice versa) with different sub-circuit modules.
We encode all single-stage Op-Amps and sub-circuit modules as functional sub-structures by using their behavioral models~\citep{topology_con}.
In this way, each functional sub-structures can be significantly simplified without using its complex exact circuit structure.
For instance, a single-stage Op-Amp with tens of transistors can be modeled as a voltage-controlled current source (VCCS, $g_m$) with a pair of parasitic capacitor $C$ and resistor $R$.
Instead of using these functional sub-structures as graph vertices, we leverage them as our graph edges while the connection point (e.g., node $1$ and node $2$) between these sub-structures is taken as vertices.
Meanwhile, we unify both feedforward and feedback directions as feedforward directions but distinguish them by adding a polarity (e.g., `$+$' for feedforward and `$-$' for feedback) on device parameters (e.g., $g_m+$ or $g_m-$). 
In this way, an arbitrary Op-Amp can be efficiently converted into an acyclic graph as shown in Figure~\ref{fig:over_arcg}.
Inversely, a newly generated circuit topology can be converted back into the corresponding Op-Amp by using the decoding process from the graph and functional sub-structures to real circuits.

\textbf{Interacting with Circuit Simulators}
Another important feature of our circuit benchmark is that it can directly interact with a circuit simulator to evaluate the performance of a generated Op-Amp in real-time.
Once a circuit topology is generated from our learning framework, a tailored Python script is used to translate it into a circuit netlist.
A circuit netlist is a standard hardware description of a circuit, based on which the circuit simulator can perform a simulation (evaluation) to extract the circuit specifications, e.g., gain, phase margin, and bandwidth for Op-Amps.
This entire process can be inherently integrated into a Python environment as both open-sourced and commercial circuit simulators support command-line operations.
%without Graphic User Interface.
We leverage the set-up to generate $10,000$ different Op-Amps with detailed circuit specifications.
Note that in our benchmark, the topologies of Op-Amps are not distinct from each other. 
Some Op-Amps have the same topology but with different device parameters.
However, our benchmark is also friendly to augment other analog circuits such as filters if the corresponding circuit-graph mapping methods are built.

==> checklist.tex <==
The main theoretical contribution of our paper comes from Lemma ~\ref{lemma:2_4}, Lemma ~\ref{lemma:2_3}, Lemma ~\ref{lemma:3_4} and Theorem ~\ref{theo:3_2}. The complete proofs of these theoretical results are available in Appendix ~\ref{sec:appenC}, Appendix ~\ref{sec:appenD} and Appendix ~\ref{sec:appenE}.  We introduce and compare datasets used in the paper in Appendix~\ref{sec:appenA}, and provide open-source code in supplementary material, including the implementation of GC-GNN as well as UGC-GNN. Graph canonization algorithms are implemented in the environment of python. Our source code to implement experiments is also provided in the supplementary materials, and we will make it public on Github in the future.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

